Line-Intensity Mapping: 2017 Status Report

Following the first two annual intensity mapping workshops at Stanford in March 2016 and Johns Hopkins in June 2017, we report on the recent advances in theory, instrumentation and observation that were presented in these meetings and some of the opportunities and challenges that were identified looking forward. With preliminary detections of CO, [CII], Lya and low-redshift 21cm, and a host of experiments set to go online in the next few years, the field is rapidly progressing on all fronts, with great anticipation for a flood of new exciting results. This current snapshot provides an efficient reference for experts in related fields and a useful resource for nonspecialists. We begin by introducing the concept of line-intensity mapping and then discuss the broad array of science goals that will be enabled, ranging from the history of star formation, reionization and galaxy evolution to measuring baryon acoustic oscillations at high redshift and constraining theories of dark matter, modified gravity and dark energy. After reviewing the first detections reported to date, we survey the experimental landscape, presenting the parameters and capabilities of relevant instruments such as COMAP, mmIMe, AIM-CO, CCAT-p, TIME, CONCERTO, CHIME, HIRAX, HERA, STARFIRE, MeerKAT/SKA and SPHEREx. Finally, we describe recent theoretical advances: different approaches to modeling line luminosity functions, several techniques to separate the desired signal from foregrounds, statistical methods to analyze the data, and frameworks to generate realistic intensity map simulations.

==> tcilcomm.tex <==
% Macros used for TCI styles released with Scientific Word 1.1.
%Copyright (C) 1992-93 TCI Software Research, Inc.
\typeout{TCILCOMM Macros for TCI styles <08 Apr 93>.}
%
% Revisions:
% 08 Apr 93 - GP change line length to under 80 characters
% 30 Mar 92 - AO added \setmoremathsizes and hooks to, e.g. \@xpt,
%             for support of bold Greek
%
%%ltg added this to try to get 12pt to come through
%\DeclareOption{12pt}{\renewcommand\@ptsize{2}}
%%end ltg

\def\@ptoptions{%
 \let\@elt\relax\@for\@tempa:=\@optionlist\do{%
  \expandafter\let\expandafter\@tempb\csname ds@\@tempa\endcsname
  \expandafter\let\expandafter\@tempc\csname ds@11pt\endcsname
  \ifx\@tempb\@tempc\else
   \expandafter\let\expandafter\@tempc\csname ds@12pt\endcsname
   \ifx\@tempb\@tempc\else\let\@tempb\relax\fi
   \fi
  \@tempb
  }%
 }%
%
% read in style file, but only process the pt size options
%
\def\@ptoptinput#1{%
 \let\@save@optionlist\@optionlist
 \let\@save@options\@options
 \let\@options\@ptoptions
 %
 \input #1
 %
 \let\@optionlist\@save@optionlist
 \let\@options\@save@options
 }%
%
% the <21 Feb 92> version of letter.sty requires:
\ifx\undefined\reset@font
 \def\reset@font{}%
 \fi
%
% Change LaTeX
%
% Add command to append tokens
\newtoks\@temptokenb
\long\def\appdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokena\the\@temptokenb}%
 }%
\long\def\prepdef#1#2{%
 \ifx#1\undefined\let#1\@empty\fi
 \@temptokena\expandafter{#1}\@temptokenb{#2}%
 \edef#1{\the\@temptokenb\the\@temptokena}%
 }%
% Discard contents of \box\@cclv at beginning of document
\appdef\document{{\output{\setbox\z@\box\@cclv}\endgraf\null\eject}}%
% Fix mark register expansion
\def\leftmark{\expandafter\@leftmark\botmark{}{}{}\@nil}%
\def\rightmark{\expandafter\@rightmark\firstmark{}{}{}\@nil}%
\def\@leftmark#1#2#3\@nil{#1}%
\def\@rightmark#1#2#3\@nil{#2}%
%
%\show\raggedright
\newskip\raggedglue
\raggedglue\z@ plus20\p@ minus\z@
\def\raggedright{%
 \let\\=\@centercr\@rightskip\raggedglue\rightskip
 \@rightskip\leftskip\z@\parindent\z@
 }%
%
\def\@centercr{%
 \ifhmode\unskip\else\@badcrerr\fi\@@par
 \@ifstar{\penalty\@M\@xcentercr}{\@xcentercr}%
 }%
%
\def\traceoutput{\tracingoutput2\showboxbreadth\maxdimen
 \showboxdepth\maxdimen}%
%
\newcount\@hour\newcount\@minute\chardef\@x10\chardef\@xv60
\def\@time{%
  \@minute\time\@hour\@minute\divide\@hour\@xv
  \ifnum\@hour<\@x 0\fi\the\@hour:%
  \multiply\@hour\@xv\advance\@minute-\@hour
  \ifnum\@minute<\@x 0\fi\the\@minute
  }%
%
% change \@array to allow \par to mean something within its scope
%
\def\@array [#1]#2{%
 \setbox\@arstrutbox\hbox{\vrule height\arraystretch\ht
  \strutbox depth\arraystretch\dp\strutbox width\z@}%
 \@mkpream{#2}%
 \edef\@preamble{\halign\noexpand\@halignto\bgroup\tabskip
  \z@\@arstrut\@preamble\tabskip\z@\cr}%
 \let\@startpbox\@@startpbox\let\@endpbox\@@endpbox
 \if#1t\vtop\else\if#1b\vbox\else\vcenter\fi\fi
 \bgroup
  %\let\par\relax
  \let\@sharp##
  \let\protect\relax
  \lineskip\z@\baselineskip\z@
  \@preamble
 }%
%
% Expands to hex digit corresponding to the value of the argument
%
\def\hexnumber@#1{\ifnum#1<10 \number#1\else
 \ifnum#1=10 A\else\ifnum#1=11 B\else\ifnum#1=12 C\else
 \ifnum#1=13 D\else\ifnum#1=14 E\else\ifnum#1=15 F\fi\fi\fi\fi\fi\fi\fi}%
%
% define command to set more math sizes.
% Styles like Greekbf will hook in here.
%
\def\setmoremathsizes#1#2#3{}%
%
% define size switch addenda
%  Note: these choices agree with those in lfonts.tex, even if incorrect.
%
\prepdef\@vpt{\setmoremathsizes{fiv}{fiv}{fiv}}%
\prepdef\@vipt{\setmoremathsizes{six}{six}{six}}%
\prepdef\@viipt{\setmoremathsizes{sev}{fiv}{fiv}}%
\prepdef\@viiipt{\setmoremathsizes{egt}{six}{fiv}}%
\prepdef\@ixpt{\setmoremathsizes{nin}{six}{fiv}}%
\prepdef\@xpt{\setmoremathsizes{ten}{sev}{fiv}}%
\prepdef\@xipt{\setmoremathsizes{elv}{egt}{six}}%
\prepdef\@xiipt{\setmoremathsizes{twl}{egt}{six}}%
\prepdef\@xivpt{\setmoremathsizes{frtn}{ten}{sev}}%
\prepdef\@xviipt{\setmoremathsizes{svtn}{twl}{ten}}%
\prepdef\@xxpt{\setmoremathsizes{twty}{frtn}{twl}}%
\prepdef\@xxvpt{\setmoremathsizes{twty}{twty}{svtn}}%
%
% The \newfield command defines (like \newenvironment) a user syntax:
%
%   \newfield{foo}
%
% lets you write
%
%   \begin{foo}...\end{foo}
%
% but differs from \newenvironment in that TeX parses the entire content
% of the field and stores it in a macro \the@foo, and then executes \@do@foo.
%
% This means that the content of the field is actually more like an argument
% than the content of an environment. So \verb will not necessarily work
% within a field, and neither will \index. Caveat emptor.
%
% The default procedure for a field is to process its argument within a
% group.  If you want a field to simply store its data away, define its
% procedure to be synonymous with \@empty, as illustrated below.
%
\long\def\@readenvir#1#2\end{%
 \appdef\envirsofar{#2}%
 \@ifnextchar\bgroup{\@checkenvir{#1}}{\@envirenderr}%
 }%
%
\def\@envirenderr{%
 \@latexerr{\string\end\space not followed by environment name}\@eha
 }%
%
\def\@checkenvir#1#2{%
 \def\@tempa{#1}\def\@tempb{#2}%
 \ifx\@tempa\@tempb
  \ifx\envirsofar\@blankspace\let\envirsofar\@empty\fi
  \expandafter\let\csname the@#1\endcsname\envirsofar
  \def\@tempa{\csname @do@#1\endcsname}%
  \else
  \appdef\envirsofar{\end{#2}}%
  \def\@tempa{\@readenvir{#1}}%
  \fi
 \@tempa
 }%
%
\def\newfield#1#2{%
 \expandafter\@ifdefinable\csname#1\endcsname{%
  \expandafter\def\csname#1\endcsname{%
   \endgroup\let\envirsofar\@empty\@readenvir{#1}%
   }%
  \expandafter\let\csname the@#1\endcsname\@empty
  \expandafter\ifx\csname @do@#1\endcsname\relax
   \expandafter\def\csname @do@#1\endcsname{{\csname the@#1\endcsname}}%
   \fi
  }%
 }%
%
\def\@blankspace{ }% SciWord's nil field
%
\def\letparBL{\def\par{\\}}%
\def\letparSP{\def\par{\ }}%
\def\letparQD{\def\par{\quad}}%
\def\letparSL{\def\par{\hbox to1em{\hfil/\hfil}}}%
%
% When \par is processed in the page head, gobble up the rest of the
% argument.
\def\@gobblepar#1\@empty{}%
%
% Physical page size after trim
\newdimen\trimwidth
\newdimen\trimheight
\newdimen\botmargin
\newdimen\marginpartotal
%
\def\adjustpagemargin{% adjust \oddsidemargin by \marginpartotal
 \marginpartotal\marginparwidth\advance\marginpartotal\marginparsep
 \advance\oddsidemargin\marginpartotal
 }%
%
\def\settextheight{% calculate textheight constrained by:
 \textheight\trimheight
 \advance\textheight-\topmargin
 \advance\textheight-\headheight
 \advance\textheight-\headsep
 \advance\textheight-\footskip
 \advance\textheight-\botmargin
 }%
%
\def\vcenterpagemargin{% calculate \topmargin constrained by:
 \topmargin\trimheight
 \advance\topmargin-\textheight
 \advance\topmargin-\headheight
 \advance\topmargin-\headsep
 \advance\topmargin-\footskip
 \divide\topmargin\tw@\botmargin\topmargin
 }%
%
\def\centerpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \divide\oddsidemargin\tw@
 \evensidemargin\oddsidemargin
 \adjustpagemargin
 }%
%
\def\leftpagemargin{% calculate \oddsidemargin constrained by:
 \oddsidemargin\trimwidth
 \advance\oddsidemargin-\textwidth
 \advance\oddsidemargin-\marginparwidth
 \advance\oddsidemargin-\marginparsep
 \advance\oddsidemargin-\evensidemargin
 \adjustpagemargin
 }%

